Exponential Communication Separations between Notions of Selfishness

We consider the problem of implementing a fixed social choice function between multiple players (which takes as input a type $t_i$ from each player $i$ and outputs an outcome $f(t_1,\ldots, t_n)$), in which each player must be incentivized to follow the protocol. In particular, we study the communication requirements of a protocol which: (a) implements $f$, (b) implements $f$ and computes payments that make it ex-post incentive compatible (EPIC) to follow the protocol, and (c) implements $f$ and computes payments in a way that makes it dominant-strategy incentive compatible (DSIC) to follow the protocol. We show exponential separations between all three of these quantities, already for just two players. That is, we first construct an $f$ such that $f$ can be implemented in communication $c$, but any EPIC implementation of $f$ (with any choice of payments) requires communication $\exp(c)$. This answers an open question of [FS09, BBS13]. Second, we construct an $f$ such that an EPIC protocol implements $f$ with communication $C$, but all DSIC implementations of $f$ require communication $\exp(C)$.

==> Conclusion.tex <==
\section{Conclusion and related directions}

We studied the 

\paragraph{Separations for practical problems}


% \paragraph{Weaker notions of incentive compatibility}
% For notions of incentive compatibility weaker than EPIC,
% one can typically ignore the extensive form game of the mechanism
% and focus solely on the protocol used to compute the social choice 
% function and transfers.
% Thus, determining the separation in the communication requirements amounts
% to simply determining the communication complexity of the
% easiest-to-compute price function which incentivize the social choice
% function.
% 
% To the best of our knowledge, the notion of ``truthful in expectation'',
% which is intermediate between EPIC and BIC, has not yet been considered in
% this context.


\paragraph{Stronger notions of incentive compatibility}
While the themes of this paper have been addressed a few times
for notions of incentive compatibility weaker than EPIC, less work
has been done for cases stronger than EPIC, where the extensive for
game the mechanism uses becomes important. 

